Evaluating Large Language Models in Detecting Test Smells

Test smells are coding issues that typically arise from inadequate practices, a lack of knowledge about effective testing, or deadline pressures to complete projects. The presence of test smells can negatively impact the maintainability and reliability of software. While there are tools that use advanced static analysis or machine learning techniques to detect test smells, these tools often require effort to be used. This study aims to evaluate the capability of Large Language Models (LLMs) in automatically detecting test smells. We evaluated ChatGPT-4, Mistral Large, and Gemini Advanced using 30 types of test smells across codebases in seven different programming languages collected from the literature. ChatGPT-4 identified 21 types of test smells. Gemini Advanced identified 17 types, while Mistral Large detected 15 types of test smells. Conclusion: The LLMs demonstrated potential as a valuable tool in identifying test smells.

==> sections/2-test-smell.tex <==
\section{Test Smells}
\label{sec:test-smell}

Researchers have coined the term test smells to describe potential design problems in test code, analogous to the ``code smells'' found in poorly designed source code~\cite{van2001refactoring,beck}. 
%Investigations on the design of test code were originally pointed out by Beck~\cite{beck}. 
These symptoms can cause tests to exhibit erratic behavior, such as flakiness, false positives, and false negatives, compromising software quality due to their limited defect-catching capabilities. Despite the concept of test smells not being new, some studies have shown that they are prevalent in both open-source and industry projects, and they negatively impact code maintenance and understanding activities~\cite{bavota2015test,van2007detection,Peruma2019Distribution}.
\citet{van2001refactoring} and \citet{mesaros} defined catalogs of test smells along with their refactoring actions.

%test smells are potential coding issues related to the implementation of automated software testing~\cite{SoaresAORGSMSFB23,van2001refactoring}. 
There are various types of test smells, which can be characterized by code duplication (\textit{Duplicated Assert})~\cite{Peruma2019Distribution}, complexity in conditional structures, lack of documentation of assertions (\textit{Assertion Roulette}), non-deterministic execution behavior~\cite{palomba2020}, among others. Test smells can condition future difficulties in the maintenance process~\cite{SoaresAORGSMSFB23}, as the incidence of test smells in the code base will impair the comprehensibility of the implemented structures as the software evolves~\cite{junior2020survey,junior2021}.

% exemplo
Listing~\ref{lst:example-magic} presents an example of the \textit{Magic Numbers} test smell. This smell occurs when a test method contains inexplicable and undocumented numeric values as parameters or values for identifiers.
%explicação
The numbers \texttt{15.5D}, \texttt{15} and \texttt{15.5D} are magic numbers, since there is no indication of their semantics in the test code.

\begin{lstlisting}[basicstyle=\footnotesize, language=Java, label=lst:example-magic, caption=Example code with \textit{Magic Numbers Test.}]
@Test
public void testGetLocalTimeAsCalendar() {
  Calendar localTime = calc.getLocalTimeAsCalendar(BigDecimal.valueOf(15.5D), Calendar.getInstance());
  assertEquals(15,localTime.get(Calendar.HOUR_OF_DAY));
  assertEquals(30,localTime.get(Calendar.MINUTE));
}
\end{lstlisting}



% As another example, the test smell \textit{Assertion Roulette} is characterized by the occurrence of multiple undocumented assertions in the test method~\cite{Santana2024}. It is identified when several assertion statements do not have a descriptive message about what is being verified. In the code example presented in Listing~\ref{lst:example-assertion-roulette}, the smell \textit{Assertion Roulette} is defined in the code snippet of the method \texttt{test\_flight}.
% The smell \textit{Assertion Roulette} exists due to the occurrence of three assertions defined in the test without explicit explanation of what each assertion represents in the verification process. This issue can hinder understanding of the context or purpose of the assertion in failure scenarios.

% \begin{lstlisting}[basicstyle=\footnotesize,  label=lst:example-assertion-roulette, language=Python, caption=Example code with \textit{Assertion Roulette.}]
% class TestFlight(unittest.TestCase):
%   def test_flight(self):
%     flight = Flight('2569',1000)
%     self.assertEqual(flight.mileage,1000)
%     self.assertTrue(flight.fullFuel)
%     self.assertTrue(flight.isValidAirLineCode())
% \end{lstlisting}

Recent studies~\cite{kim2021, panichella2022, SoaresRGAS23, pontillo2024, Santana2024} have investigated the impact of test smells~\cite{campos2021} and how these indicators of poor coding affect the comprehension and quality of software~\cite{spadini2018}. 
%Discussions about the risks associated with the presence of test smells to software reliability are directed towards planning and improving tools that can detect and automate code refactorings.
%llms
However, to the best of our knowledge, no study so far indicates to what extent LLMs can help detect test smells.
%Understanding the potential of LLMs in natural language processing tasks reveals a valuable resource that can be applied to code analysis and integrated into test smell detection tools, making the code review process more robust through the automation of reading and refactoring structures in source code. 

